Predicting Program Exit Code with LLMs and Programming Language Semantics

Large language models (LLMs) have shown proficiency in various software engineering tasks, such as code generation and translation. However, a key limitation in their performance may be their (lack of) understanding of programming-language semantics. Even when explicit semantics are given, it remains unclear whether LLMs apply those rules or lean on priors learned during pre-training instead. We study if LLMs lean on priors or given semantics with a novel task--Program Executability Prediction (PrEx)--that asks models to predict whether a program is semantically valid or invalid (and, if invalid, which formal rule it violates) given the program's syntax and operational semantics. Because PrEx requires both valid and invalid programs, we build a dataset with systematically generated invalid transformations derived from valid programs. We evaluate open-source coding LLMs under two semantic formalisms and two semantic shifts across Human-Written, LLM-Translated, and Fuzzer-Generated program splits. Our findings show that LLMs lean on pre-training priors rather than systematically applying the given rules, performing especially poorly on modified semantics and degrading further as program complexity increases. PrEx is available at https://github.com/EngineeringSoftware/prex.

==> figures/pep-task-example-listings/invalid-content.tex <==
\begin{PEPProgramBox}
\PEPProgramLine{1}{int i;}
\PEPProgramLine{2}{int ans;}
\PEPProgramLine{3}{int n;}
\PEPProgramLine{4}{i = 1;}
\PEPProgramLine{5}{n = 10;}
\PEPProgramLine{6}{while ((i * i) <= n) \{}
\PEPProgramLineIndent{7}{\PEPHighlightError{n = 0;}}
\PEPProgramLineIndent{8}{i = ((i \PEPHighlightError{/ n}) + 1);}
\PEPProgramLineIndent{9}{ans = (ans + 1);}
\PEPProgramLine{10}{\};}
\end{PEPProgramBox}


==> figures/pep-task-example-listings/valid-content.tex <==
\begin{PEPProgramBox}
\PEPProgramLine{1}{int i;}
\PEPProgramLine{2}{int ans;}
\PEPProgramLine{3}{int n;}
\PEPProgramLine{4}{i = 1;}
\PEPProgramLine{5}{n = 10;}
\PEPProgramLine{6}{while ((i * i) <= n) \{}
\PEPProgramLineIndent{7}{i = (i + 1);}
\PEPProgramLineIndent{8}{ans = (ans + 1);}
\PEPProgramLine{9}{\};}
\end{PEPProgramBox}


==> figures/pep-task-example_styles.tex <==
\usetikzlibrary{positioning}

\newcommand{\pepStatusIconCheck}{%
    \tikz[baseline=(current bounding box.center)]{%
        \draw[white, line width=3.4pt, line cap=butt, line join=miter]
            (-0.16,-0.02) -- (-0.05,-0.13) -- (0.18,0.12);%
    }%
}

\newcommand{\pepStatusIconCross}{%
    \tikz[baseline=(current bounding box.center)]{%
        \draw[white, line width=3.4pt, line cap=butt, line join=miter]
            (-0.12,0.12) -- (0.12,-0.12);
        \draw[white, line width=3.4pt, line cap=butt, line join=miter]
            (-0.12,-0.12) -- (0.12,0.12);%
    }%
}

\newcommand{\pepStatusIconBug}{%
    \raisebox{-0.5pt}{\scalebox{1.05}{\faIcon{bug}}}%
}

\tikzset{
    pep codecontainer/.style={
        line width=1pt,
        inner sep=4pt,
        rounded corners=2pt,
        anchor=north west
    },
    pep codecontainervalid/.style={
        pep codecontainer,
        draw=green!60!black,
        fill=white
    },
    pep codecontainerinvalid/.style={
        pep codecontainer,
        draw=red!75!black,
        fill=white
    },
    pep statusicon/.style={
        circle,
        minimum size=0.78cm,
        inner sep=0pt,
        line width=0.7pt,
        draw=white
    },
    pep statusiconvalid/.style={
        pep statusicon,
        fill=green!60!black,
        text=white
    },
    pep statusiconinvalid/.style={
        pep statusicon,
        fill=red!70!black,
        text=white
    }
}


==> tables/numbers-pcp-IMP-K.tex <==
%% Automatically generated by: table.py make_numbers

\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-accuracy}{41}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-precision-positive}{97}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-recall-positive}{60}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-f1-positive}{74}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-precision-negative}{71}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-recall-negative}{98}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-f1-negative}{83}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-None}{40}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-Rule 2}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-Rule 31}{43}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-Rule 34}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-Rule 7}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-Rule 9}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-accuracy}{52}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-precision-positive}{93}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-recall-positive}{85}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-f1-positive}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-precision-negative}{86}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-recall-negative}{94}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-f1-negative}{90}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-malformed-count}{33.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-None}{15}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-Rule 2}{92}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-Rule 31}{38}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-Rule 34}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-Rule 7}{84}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-Rule 9}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-accuracy}{40}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-precision-positive}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-recall-positive}{48}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-f1-positive}{65}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-precision-negative}{66}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-recall-negative}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-f1-negative}{79}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-None}{52}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-Rule 2}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-Rule 31}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-Rule 34}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-Rule 7}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-Rule 9}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-accuracy}{56}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-precision-positive}{96}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-recall-positive}{79}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-f1-positive}{87}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-precision-negative}{82}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-recall-negative}{97}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-f1-negative}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-malformed-count}{10.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-None}{21}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-Rule 2}{88}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-Rule 31}{17}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-Rule 34}{78}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-Rule 7}{66}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-Rule 9}{98}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-accuracy}{58}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-precision-positive}{59}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-recall-positive}{97}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-f1-positive}{73}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-precision-negative}{92}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-recall-negative}{33}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-f1-negative}{49}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-None}{3}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-Rule 2}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-Rule 31}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-Rule 34}{97}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-Rule 7}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-Rule 9}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-accuracy}{63}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-precision-positive}{58}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-recall-positive}{93}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-f1-positive}{72}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-precision-negative}{84}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-recall-negative}{33}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-f1-negative}{47}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-malformed-count}{6.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-None}{7}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-Rule 2}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-Rule 31}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-Rule 34}{71}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-Rule 7}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-Rule 9}{66}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-accuracy}{65}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-precision-positive}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-recall-positive}{91}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-f1-positive}{95}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-precision-negative}{92}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-recall-negative}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-f1-negative}{96}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-malformed-count}{4.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-None}{9}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-Rule 2}{73}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-Rule 31}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-Rule 34}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-Rule 7}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-Rule 9}{85}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-accuracy}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-precision-positive}{59}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-recall-positive}{96}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-f1-positive}{73}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-precision-negative}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-recall-negative}{33}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-f1-negative}{48}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-malformed-count}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-None}{4}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-Rule 2}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-Rule 31}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-Rule 34}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-Rule 7}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-Rule 9}{65}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-Rule 9-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-accuracy}{30}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-accuracy-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-precision-positive}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-precision-positive-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-recall-positive}{49}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-recall-positive-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-f1-positive}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-f1-positive-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-precision-negative}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-precision-negative-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-recall-negative}{51}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-recall-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-f1-negative}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-f1-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-malformed-count}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-malformed-count-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-None}{51}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-None-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-Rule 2}{91}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-Rule 2-std}{4}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-Rule 31}{89}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-Rule 31-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-Rule 34}{91}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-Rule 34-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-Rule 7}{90}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-Rule 7-std}{3}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-Rule 9}{89}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-Rule 9-std}{4}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-accuracy}{21}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-positive}{95}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-positive}{22}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-positive}{36}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-negative}{56}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-negative}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-negative}{71}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-None}{78}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 2}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 31}{21}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 34}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 7}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 9}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-accuracy}{18}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-positive}{91}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-positive}{33}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-positive}{48}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-negative}{59}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-negative}{97}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-negative}{73}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-None}{67}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 2}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 31}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 34}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 7}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 9}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-accuracy}{42}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-positive}{87}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-positive}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-positive}{78}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-negative}{75}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-negative}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-negative}{82}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-malformed-count}{38.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-None}{30}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 2}{92}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 31}{54}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 34}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 7}{95}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 9}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-accuracy}{35}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-positive}{46}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-positive}{66}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-positive}{54}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-negative}{41}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-negative}{23}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-negative}{30}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-malformed-count}{71.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-None}{34}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 2}{88}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 31}{92}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 34}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 7}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 9}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-accuracy}{17}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-positive}{95}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-positive}{9}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-positive}{16}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-negative}{52}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-negative}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-negative}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-None}{91}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 2}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 31}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 34}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 7}{97}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 9}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-accuracy}{13}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-positive}{82}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-positive}{7}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-positive}{12}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-negative}{51}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-negative}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-negative}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-None}{93}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 2}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 31}{23}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 34}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 7}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 9}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-accuracy}{51}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-positive}{90}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-positive}{72}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-positive}{80}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-negative}{77}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-negative}{92}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-negative}{84}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-malformed-count}{8.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-None}{28}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 2}{82}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 31}{9}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 34}{80}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 7}{91}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 9}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-accuracy}{50}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-positive}{71}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-positive}{81}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-positive}{75}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-negative}{78}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-negative}{67}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-negative}{72}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-malformed-count}{29.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-None}{19}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 2}{82}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 31}{94}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 34}{51}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 7}{81}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 9}{92}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-accuracy}{30}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-positive}{39}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-positive}{47}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-positive}{43}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-negative}{34}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-negative}{28}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-negative}{31}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-None}{53}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 2}{76}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 31}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 34}{98}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 7}{95}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 9}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-accuracy}{52}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-positive}{52}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-positive}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-positive}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-negative}{95}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-negative}{8}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-negative}{15}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-None}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 2}{93}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 31}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 34}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 7}{85}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 9}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-accuracy}{48}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-positive}{49}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-positive}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-positive}{57}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-negative}{48}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-negative}{29}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-negative}{36}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-malformed-count}{5.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-None}{31}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 2}{72}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 31}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 34}{72}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 7}{94}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 9}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-accuracy}{58}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-positive}{55}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-positive}{90}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-positive}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-negative}{73}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-negative}{27}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-negative}{40}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-malformed-count}{2.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-None}{10}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 2}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 31}{79}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 34}{81}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 7}{66}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 9}{71}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-accuracy}{26}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-positive}{96}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-positive}{14}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-positive}{25}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-negative}{54}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-negative}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-negative}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-None}{86}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 2}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 31}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 34}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 7}{81}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 9}{74}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-accuracy}{60}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-positive}{83}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-positive}{95}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-positive}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-negative}{95}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-negative}{81}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-negative}{87}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-None}{5}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 2}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 31}{22}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 34}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 7}{90}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 9}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-accuracy}{45}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-positive}{47}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-positive}{61}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-positive}{53}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-negative}{44}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-negative}{31}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-negative}{36}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-malformed-count}{9.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-None}{39}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 2}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 31}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 34}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 7}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 9}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-Rule 9-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-accuracy}{59}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-positive}{55}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-positive}{97}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-positive}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-negative}{88}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-negative}{21}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-negative}{34}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-None}{3}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 2}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 31}{94}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 31-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 34}{96}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 34-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 7}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 7-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 9}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-Rule 9-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-accuracy}{30}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-accuracy-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-precision-positive}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-recall-positive}{49}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-recall-positive-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-f1-positive}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-f1-positive-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-precision-negative}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-recall-negative}{51}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-recall-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-f1-negative}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-f1-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-malformed-count}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-None}{51}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-None-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-Rule 2}{91}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-Rule 2-std}{4}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-Rule 31}{89}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-Rule 31-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-Rule 34}{91}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-Rule 34-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-Rule 7}{90}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-Rule 7-std}{3}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-Rule 9}{89}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-Rule 9-std}{4}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-accuracy}{31}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-accuracy-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-precision-positive}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-precision-positive-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-recall-positive}{51}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-recall-positive-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-f1-positive}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-f1-positive-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-precision-negative}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-precision-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-recall-negative}{49}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-recall-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-f1-negative}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-f1-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-malformed-count}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-malformed-count-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-None}{49}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-None-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-Rule 2}{93}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-Rule 2-std}{3}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-Rule 31}{85}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-Rule 31-std}{4}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-Rule 34}{89}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-Rule 34-std}{4}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-Rule 7}{87}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-Rule 7-std}{3}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-Rule 9}{87}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-Rule 9-std}{2}


==> tables/numbers-pcp-IMP-SOS.tex <==
%% Automatically generated by: table.py make_numbers

\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-accuracy}{60}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-precision-positive}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-recall-positive}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-f1-positive}{94}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-precision-negative}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-recall-negative}{88}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-f1-negative}{93}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-None}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-Rule 19}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-Rule 2}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-Rule 23}{96}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-Rule 73}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-Rule 76}{21}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-accuracy}{55}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-precision-positive}{96}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-recall-positive}{83}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-f1-positive}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-precision-negative}{85}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-recall-negative}{96}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-f1-negative}{90}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-malformed-count}{50.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-None}{17}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-Rule 19}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-Rule 2}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-Rule 23}{87}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-Rule 73}{92}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-Rule 76}{14}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-accuracy}{46}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-precision-positive}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-recall-positive}{54}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-f1-positive}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-precision-negative}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-recall-negative}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-f1-negative}{81}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-None}{46}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-Rule 19}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-Rule 2}{91}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-Rule 23}{73}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-Rule 73}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-Rule 76}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-accuracy}{58}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-precision-positive}{96}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-recall-positive}{78}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-f1-positive}{86}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-precision-negative}{81}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-recall-negative}{96}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-f1-negative}{88}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-malformed-count}{5.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-None}{22}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-Rule 19}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-Rule 2}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-Rule 23}{78}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-Rule 73}{94}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-Rule 76}{17}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-accuracy}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-precision-positive}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-recall-positive}{96}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-f1-positive}{98}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-precision-negative}{96}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-recall-negative}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-f1-negative}{98}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-None}{4}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-Rule 19}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-Rule 2}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-Rule 23}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-Rule 73}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-Rule 76}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-accuracy}{63}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-precision-positive}{59}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-recall-positive}{95}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-f1-positive}{73}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-precision-negative}{87}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-recall-negative}{33}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-f1-negative}{48}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-malformed-count}{2.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-None}{5}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-Rule 19}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-Rule 2}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-Rule 23}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-Rule 73}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-Rule 76}{72}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-accuracy}{66}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-precision-positive}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-recall-positive}{85}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-f1-positive}{92}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-precision-negative}{87}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-recall-negative}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-f1-negative}{93}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-None}{15}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-Rule 19}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-Rule 2}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-Rule 23}{71}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-Rule 73}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-Rule 76}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-accuracy}{61}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-precision-positive}{58}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-recall-positive}{92}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-f1-positive}{71}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-precision-negative}{80}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-recall-negative}{34}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-f1-negative}{47}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-malformed-count}{5.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-None}{8}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-Rule 19}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-Rule 2}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-Rule 23}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-Rule 73}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-Rule 76}{78}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-Rule 76-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-accuracy}{30}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-accuracy-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-precision-positive}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-precision-positive-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-recall-positive}{49}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-recall-positive-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-f1-positive}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-f1-positive-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-precision-negative}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-precision-negative-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-recall-negative}{51}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-recall-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-f1-negative}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-f1-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-malformed-count}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-malformed-count-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-None}{51}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-None-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-Rule 19}{90}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-Rule 19-std}{3}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-Rule 2}{91}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-Rule 2-std}{4}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-Rule 23}{89}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-Rule 23-std}{4}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-Rule 73}{91}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-Rule 73-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-Rule 76}{89}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-Rule 76-std}{1}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy}{58}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-positive}{87}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-positive}{94}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-positive}{90}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-negative}{93}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-negative}{86}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-negative}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-None}{6}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 19}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 2}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 23}{94}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 73}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 76}{13}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-accuracy}{50}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-positive}{75}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-positive}{81}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-positive}{78}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-negative}{80}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-negative}{74}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-negative}{77}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-None}{19}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 19}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 2}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 23}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 73}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 76}{25}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-accuracy}{46}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-positive}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-positive}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-positive}{77}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-negative}{74}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-negative}{91}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-negative}{82}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-malformed-count}{48.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-None}{32}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 19}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 2}{91}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 23}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 73}{90}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 76}{17}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-accuracy}{40}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-positive}{63}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-positive}{72}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-positive}{67}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-negative}{67}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-negative}{58}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-negative}{62}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-malformed-count}{89.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-None}{28}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 19}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 2}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 23}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 73}{58}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 76}{98}
\DefMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy}{22}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-positive}{93}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-positive}{14}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-positive}{24}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-negative}{53}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-negative}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-negative}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-None}{86}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 19}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 2}{91}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 23}{76}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 73}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 76}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-accuracy}{16}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-positive}{86}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-positive}{6}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-positive}{11}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-negative}{51}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-negative}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-negative}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-None}{94}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 19}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 2}{85}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 23}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 73}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 76}{1}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-accuracy}{52}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-positive}{88}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-positive}{74}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-positive}{80}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-negative}{78}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-negative}{90}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-negative}{83}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-malformed-count}{5.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-None}{26}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 19}{95}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 2}{77}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 23}{81}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 73}{95}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 76}{17}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-accuracy}{48}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-positive}{73}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-positive}{79}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-positive}{76}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-negative}{77}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-negative}{71}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-negative}{74}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-malformed-count}{14.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-None}{21}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 19}{98}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 2}{74}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 23}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 73}{36}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 76}{98}
\DefMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy}{43}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-positive}{90}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-positive}{43}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-positive}{58}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-negative}{62}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-negative}{95}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-negative}{75}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-None}{57}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 19}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 2}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 23}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 73}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 76}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-accuracy}{53}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-positive}{52}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-positive}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-positive}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-negative}{88}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-negative}{9}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-negative}{16}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-None}{1}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 19}{84}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 2}{72}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 23}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 73}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 76}{98}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-accuracy}{47}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-positive}{51}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-positive}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-positive}{59}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-negative}{52}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-negative}{34}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-negative}{42}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-malformed-count}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-None}{31}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 19}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 2}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 23}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 73}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 76}{72}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-accuracy}{59}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-positive}{78}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-positive}{91}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-positive}{84}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-negative}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-negative}{74}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-negative}{81}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-malformed-count}{11.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-None}{9}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 19}{72}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 2}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 23}{72}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 73}{41}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 76}{100}
\DefMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy}{34}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-positive}{92}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-positive}{24}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-positive}{38}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-negative}{56}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-negative}{98}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-negative}{71}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-None}{76}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 19}{89}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 2}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 23}{66}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 73}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 76}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-accuracy}{54}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-positive}{91}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-positive}{77}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-positive}{83}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-negative}{80}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-negative}{92}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-negative}{86}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-malformed-count}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-None}{23}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 19}{77}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 2}{69}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 23}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 73}{12}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 76}{84}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-accuracy}{43}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-positive}{46}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-positive}{59}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-positive}{52}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-negative}{42}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-negative}{29}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-negative}{34}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-malformed-count}{5.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-None}{41}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 19}{94}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 2}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 23}{64}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 73}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 76}{75}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-Rule 76-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-accuracy}{57}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-accuracy-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-positive}{58}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-positive}{95}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-positive}{72}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-positive-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-negative}{87}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-precision-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-negative}{31}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-recall-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-negative}{46}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-f1-negative-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-malformed-count}{7.0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-malformed-count-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-None}{5}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-None-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 19}{70}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 19-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 2}{68}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 2-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 23}{74}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 23-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 73}{99}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 73-std}{0}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 76}{93}
\DefMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-Rule 76-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy}{30}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-precision-positive}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-precision-positive-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-recall-positive}{49}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-recall-positive-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-f1-positive}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-f1-positive-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-precision-negative}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-precision-negative-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-recall-negative}{51}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-recall-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-f1-negative}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-f1-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-malformed-count}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-malformed-count-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-None}{51}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-None-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 19}{90}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 19-std}{3}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 2}{91}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 2-std}{4}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 23}{89}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 23-std}{4}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 73}{91}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 73-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 76}{89}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-Rule 76-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-accuracy}{31}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-accuracy-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-precision-positive}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-precision-positive-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-recall-positive}{51}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-recall-positive-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-f1-positive}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-f1-positive-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-precision-negative}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-precision-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-recall-negative}{49}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-recall-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-f1-negative}{50}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-f1-negative-std}{1}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-malformed-count}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-malformed-count-std}{0}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-None}{49}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-None-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-Rule 19}{87}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-Rule 19-std}{3}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-Rule 2}{93}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-Rule 2-std}{3}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-Rule 23}{87}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-Rule 23-std}{2}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-Rule 73}{89}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-Rule 73-std}{4}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-Rule 76}{85}
\DefMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-Rule 76-std}{4}


==> tables/table-imp-split-complexity-stats.tex <==
%% Automatically generated by: table.py make_imp_split_complexity_stats_table

\TableFont
\caption{\UseMacro{TCap-imp-split-complexity-stats}}
\label{tab:imp-split-complexity-stats}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{l r r r r}
\toprule
\textbf{\UseMacro{THead-imp-split-complexity-split}} & \textbf{\UseMacro{THead-imp-split-complexity-num-programs}} & \textbf{\UseMacro{THead-imp-split-complexity-cc}} & \textbf{\UseMacro{THead-imp-split-complexity-max-nested-if}} & \textbf{\UseMacro{THead-imp-split-complexity-max-nested-while}}
\\
\midrule
\UseMacro{THead-imp-split-complexity-human-written}
 & \UseMacro{dataset-imp-split-complexity-human-written-num-programs} & \UseMacro{dataset-imp-split-complexity-human-written-median-cc} & \UseMacro{dataset-imp-split-complexity-human-written-median-max-nested-if} & \UseMacro{dataset-imp-split-complexity-human-written-median-max-nested-while}
\\
\UseMacro{THead-imp-split-complexity-synthetic-cpp}
 & \UseMacro{dataset-imp-split-complexity-synthetic-cpp-num-programs} & \UseMacro{dataset-imp-split-complexity-synthetic-cpp-median-cc} & \UseMacro{dataset-imp-split-complexity-synthetic-cpp-median-max-nested-if} & \UseMacro{dataset-imp-split-complexity-synthetic-cpp-median-max-nested-while}
\\
\UseMacro{THead-imp-split-complexity-fuzzer-generated}
 & \UseMacro{dataset-imp-split-complexity-fuzzer-generated-num-programs} & \UseMacro{dataset-imp-split-complexity-fuzzer-generated-median-cc} & \UseMacro{dataset-imp-split-complexity-fuzzer-generated-median-max-nested-if} & \UseMacro{dataset-imp-split-complexity-fuzzer-generated-median-max-nested-while}
\\
\bottomrule
\end{tabular}

==> tables/table-pcp-fuzzing-examples.tex <==
\begin{table*}[t]
  \centering
  \TableFont
  \caption{\UseMacro{TCap-pcp-fuzzing-examples}}
  \label{tab:pcp-fuzzing-examples}
  \setlength{\tabcolsep}{3pt}
  \input{figures/pcp-fuzzing-example-codes}
  \begin{tabular}{@{}>{\raggedright\arraybackslash}p{0.155\linewidth}
                       >{\raggedright\arraybackslash}p{0.155\linewidth}
                       >{\raggedright\arraybackslash}p{0.155\linewidth}
                       >{\raggedright\arraybackslash}p{0.155\linewidth}
                       >{\raggedright\arraybackslash}p{0.155\linewidth}
                       >{\raggedright\arraybackslash}p{0.155\linewidth}@{}}
    \toprule
    \multicolumn{1}{c}{\textbf{\UseMacro{THead-pcp-fuzzing-valid-group}}}
    & \multicolumn{5}{c}{\textbf{\UseMacro{THead-pcp-fuzzing-invalid-group}}} \\
    \cmidrule(lr){1-1}\cmidrule(lr){2-6}
    \textbf{\UseMacro{THead-pcp-fuzzing-valid}}
    & \textbf{\UseMacro{THead-semantic-error-break-outside-loop}}
    & \textbf{\UseMacro{THead-semantic-error-continue-outside-loop}}
    & \textbf{\UseMacro{THead-semantic-error-divide-by-zero}}
    & \textbf{\UseMacro{THead-semantic-error-modulo-zero}}
    & \textbf{\UseMacro{THead-semantic-error-var-use-before-declare}} \\
    \midrule
    \PCPFuzzLstInput{figures/pcp-fuzzing-listings/valid.tex}
    &
    \PCPFuzzLstInput{figures/pcp-fuzzing-listings/break-outside-loop.tex}
    &
    \PCPFuzzLstInput{figures/pcp-fuzzing-listings/continue-outside-loop.tex}
    &
    \PCPFuzzLstInput{figures/pcp-fuzzing-listings/divide-by-zero.tex}
    &
    \PCPFuzzLstInput{figures/pcp-fuzzing-listings/modulo-zero.tex}
    &
    \PCPFuzzLstInput{figures/pcp-fuzzing-listings/var-use-before-declare.tex}
    \\
    \bottomrule
  \end{tabular}
\end{table*}


==> tables/table-results-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder.tex <==
%% Automatically generated by: table.py make_two_results_table_same_task

\begin{table*}[t]
\begin{center}
\TableFont
\caption{\UseMacro{TCap-models-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder}\label{tab:pcp-IMP-K-IMP-SOS-accuracy-qwen-coder}}
\begin{threeparttable}
\begin{tabular}{l  c  c  c  c  c  c  c }
\toprule
\multirow{2}{*}{\textbf{\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-models}}}
& \multicolumn{3}{c}{\textbf{\Kos-semantics}}
& \multicolumn{3}{c}{\textbf{\Sos}}
\\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
 & \textbf{\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-pcp-uk-IMP-K-accuracy}}
 & \textbf{\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-pcp-mk-IMP-K-KeywordSwap-accuracy}}
 & \textbf{\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-pcp-mk-IMP-K-KeywordObf-accuracy}}
 & \textbf{\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-pcp-uk-IMP-SOS-accuracy}}
 & \textbf{\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-pcp-mk-IMP-SOS-KeywordSwap-accuracy}}
 & \textbf{\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-pcp-mk-IMP-SOS-KeywordObf-accuracy}}
\\
\midrule
\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-Qwen-Qwen2.5-Coder-3B-Instruct-da}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-K-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-K-KeywordObf-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-uk-IMP-SOS-accuracy}
 & \textbf{\UseMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy}}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-accuracy}
\\
\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-Qwen-Qwen2.5-Coder-7B-Instruct-da}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-K-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-K-KeywordObf-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-uk-IMP-SOS-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-accuracy}
\\
\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-Qwen-Qwen2.5-Coder-14B-Instruct-da}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-K-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-K-KeywordObf-accuracy}
 & \textbf{\UseMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-uk-IMP-SOS-accuracy}}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-accuracy}
\\
\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-Qwen-Qwen2.5-Coder-32B-Instruct-da}
 & \textbf{\UseMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-K-accuracy}}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordSwap-accuracy}
 & \textbf{\UseMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-K-KeywordObf-accuracy}}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-uk-IMP-SOS-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-da-pcp-mk-IMP-SOS-KeywordObf-accuracy}
\\
\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-random-guesser-dataset-distribution-da}\tnote{*}
 & \UseMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-K-accuracy}
 & \UseMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordSwap-accuracy}
 & \UseMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-K-KeywordObf-accuracy}
 & \UseMacro{res-random-guesser-dataset-distribution-da-pcp-uk-IMP-SOS-accuracy}
 & \UseMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordSwap-accuracy}
 & \UseMacro{res-random-guesser-dataset-distribution-da-pcp-mk-IMP-SOS-KeywordObf-accuracy}
\\
\midrule
\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-Qwen-Qwen2.5-Coder-3B-Instruct-cot}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-K-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-uk-IMP-SOS-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-3B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-accuracy}
\\
\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-Qwen-Qwen2.5-Coder-7B-Instruct-cot}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-K-accuracy}
 & \textbf{\UseMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-accuracy}}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-uk-IMP-SOS-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-7B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-accuracy}
\\
\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-Qwen-Qwen2.5-Coder-14B-Instruct-cot}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-K-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-uk-IMP-SOS-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-accuracy}
 & \textbf{\UseMacro{res-Qwen-Qwen2.5-Coder-14B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-accuracy}}
\\
\UseMacro{THead-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-Qwen-Qwen2.5-Coder-32B-Instruct-cot}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-K-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordSwap-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-K-KeywordObf-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-uk-IMP-SOS-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordSwap-accuracy}
 & \UseMacro{res-Qwen-Qwen2.5-Coder-32B-Instruct-cot-pcp-mk-IMP-SOS-KeywordObf-accuracy}
\\
\bottomrule
\end{tabular}
\begin{tablenotes}
\scriptsize
\item * The random guesser uses a weighted random selection based on the distribution of the dataset.
\end{tablenotes}
\end{threeparttable}
\end{center}
\end{table*}

==> tables/table-results-qwen-coder-by-split.tex <==
%% Automatically generated by: visualize_pcp_split_accuracy_tables.py
%% Combined view of all three dataset splits.
%% Macros are loaded from macros.tex via tables/macros-table-qwen-coder-by-split.tex

\input{tables/table-results-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-by-split-human-written}

\input{tables/table-results-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-by-split-llm-translated}

\input{tables/table-results-pcp-IMP-K-IMP-SOS-accuracy-qwen-coder-by-split-fuzzer-generated}

